Navigating Decision Landscapes: The Impact of Principals on Decision-Making Dynamics

We explored decision-making dynamics in social systems, referencing the 'herd behavior' from prior studies where individuals follow preceding choices without understanding the underlying reasons. While previous research highlighted a preference for the optimal choice without external influences, our study introduced principals or external guides, adding complexity to the decision-making process. The reliability of these principals significantly influenced decisions. Notably, even occasional trust in an unreliable principal could alter decision outcomes. Furthermore, when a principal's advice was purely random, heightened trust led to more decision errors. Our findings emphasize the need for caution when placing trust in decision-making contexts.

==> candidate.tex <==
\section{Data and Results}
\subsection{Decision Dynamics Uninfluenced by Principals}
\label{Decisionnoprincipal}

Decision-making dynamics, particularly in the context of social systems, often exhibit intricate behaviors. One such intriguing phenomenon is the `herd behavior.' In this behavior, as time progresses, a preponderance of participants tend to coalesce around a singular choice. Interestingly, subsequent decision-makers are privy merely to the choice itself, devoid of the underlying rationale that initially culminated in that choice.

To offer clarity on this dynamics, we configured our model with the parameters: \( \mu_A = 1 \), \( \mu_B = 0 \), \( \sigma = 1 \), and \( k = 1 \). We made an assumption wherein the objective signal is uniformly sampled from \(N(\mu_A, \sigma^2) \). This configuration bore results that were in congruence with the seminal works of \cite{GU2015471}. Specifically, a continual increase in the proportion of participants favoring choice \(A\) was evident. This is consistent with our model's architecture where the decision threshold, represented by \(r(\beta) \), gravitates incrementally towards \(\mu_B\), thereby attenuating the pertinence of the objective signal in sequential decisions.

The dynamics are lucidly illustrated in Fig.\ref{fig:Percentage_NoPrinciple}, which delineates the proportion of decision-makers allying with the correct choice, indexed by decision count. Corroborating the observations made in \cite{Browne,GU2015471}, there emerges a clear convergence pattern toward the accurate choice, intensifying with an increasing ensemble of decision-makers.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{Percentage_NoPrinciple.pdf}
    \caption{Convergence of the WB model devoid of principal influence.}
    \label{fig:Percentage_NoPrinciple}
\end{figure}

\subsection{Decision Dynamics Modulated by Always Trusted Principals}
\label{Decisiontrustedprincipal}
Incorporating principals into the decision-making landscape introduces additional complexities. Crucially, in our configuration, these principals are not guaranteed to be sources of the correct signal, denoted here as option \(A\). We employ \(p_\text{bias}\) to quantify the probability with which a principal's guidance is sculpted from the correct signal distribution \(N(\mu_A, \sigma^2)\). In the event of a deviation, the guidance conforms to the incorrect signal distribution \(N(\mu_B, \sigma^2)\).

Fig.\ref{fig:Percentage_Principle} presents a comparative analysis across diverse \(p_\text{bias}\) values. The principal's influence becomes unmistakably salient: the convergence trajectory of decision-makers appears heavily modulated by the veracity of the principal's signal. Remarkably, this sway persists even when private signals are invariably derived from \(N(\mu_A, \sigma^2)\). For a holistic comparison, the principal-exempt scenario from Sec.\ref{Decisionnoprincipal} is also exhibited.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{Percentage_Principle.pdf}
    \caption{Emergent dynamics under the P-WB model.}
    \label{fig:Percentage_Principle}
\end{figure}

A comprehensive evaluation yields several key insights:

\begin{enumerate}
    \item A principal that is predominantly accurate catalyzes a swifter convergence to the optimal decision.
    \item Conversely, a principal with frequent misdirections tends to derail decisions towards suboptimal outcomes.
    \item When the principal's accuracy exceeds a critical threshold of \(50\%\), initial convergence may be tepid, but it eventually overtakes the baseline trajectory, underscoring the principal's overarching influence.
    \item Notably, when \(p_\text{bias} = 0.5\), the decision pattern reaches a stasis, evincing no clear convergence. To further scrutinize this intriguing behavior, we extended our analysis to encompass 1000 decision events, as delineated in Fig.\ref{fig:Percentage_Principle_zoomout}. Even within this expansive horizon, a definitive convergence trend remains nebulous.
\end{enumerate}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{Percentage_Principle_zoomout.pdf}
    \caption{Prolonged observation of the P-WB model spanning 1000 decisions.}
    \label{fig:Percentage_Principle_zoomout}
\end{figure}

\subsection{Decision Dynamics Modulated by Not Always Trusted Principals}
In Sec.\ref{Decisiontrustedprincipal}, we employed a principal that is always trusted by the decision-maker, and showed that the convergence of the decision is dominated by the impact of the principal. In this section, we introduce another layer of complexity: the principal is not always trusted, regardless of its signal. In this study, We denote \(p_\text{trust}\) as the probability that the principal's signal is trusted by the decision-maker. When a principal signal is trusted, the decision-maker will move the decision boundary according to Eq.\ref{principal_decision}. When a principal signal is not trusted, the decision-maker simply will just ignore the principal signal, and update the decision boundary according to the following formula \cite{Browne}:
\begin{equation}
\beta_{t+1} = \frac{p(D_t | A_t, \mu_B)}{p(D_t | A_t, \mu_A)} \beta_t
\label{noprincipal_decision}
\end{equation}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{Percentage_Principle_trustness.pdf}
    \caption{}
    \label{fig:Percentage_Principle_trustness}
\end{figure}

For our analysis, we first compare the results with various \(p_\text{trust}\) values under \(p_\text{bias} = 0.3\). This configuration implies that the principal's guidance is correct 30\% of the time, and even then, decision-makers trust this guidance only 10\% of the time. The results, as depicted in Fig.\ref{fig:Percentage_Principle_trustness}, are intriguing. Initially, there's an uptick in the percentage of correct decisions, suggesting that the decision-makers are learning from previous correct decisionns. However, as more decisions are made, this trend reverses, and the percentage of correct decisions starts to decline. This counterintuitive outcome underscores a pivotal insight: even when a evil principal, who is predominantly misleading, is rarely trusted, its mere presence can significantly alter the trajectory of decision-making. This phenomenon can be attributed to the previous study that shows good principal's guidances reinforces the convergence towards correct decision. However, in this study, as more decisions are influenced by the principal's incorrect guidance, the overall correctness rate of decisions diminishes.

This observation resonates with the broader theme of our study, emphasizing the profound impact of external influences, such as principals, on sequential decision-making. Even when these influences are sporadic and often unreliable, they can sway the collective decision-making behavior, underscoring the need for decision-makers to be discerning in whom or what they place their trust.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{Percentage_Principle_trustness_bias.pdf}
    \caption{}
    \label{fig:Percentage_Principle_trustness_bias}
\end{figure}

In a subsequent analysis, we adjusted \(p_\text{bias}\) to 0.5, indicating that the principal's guidance is accurate 50% of the time, rendering it statistically random. Fig.\ref{fig:Percentage_Principle_trustness_halfbias} delineates the decision-making accuracy as a function of varying \(p_\text{trust}\) values. Surprisingly, an inverse relationship emerges: as trust in the principal augments, the accuracy of decisions diminishes. This observation posits that heightened trust in a statistically random principal can inadvertently divert decision-makers from optimal outcomes.

A preliminary assumption might posit a neutral influence of a random principal on decision-making. Yet, the data suggests that the act of conferring trust in an external source, even if its guidance is statistically random, can infuse variability into the decision-making trajectory. This variability, when aggregated over a sequence of decisions, can deviate from optimal decision pathways.

This analysis accentuates the intricate relationship between trust and decision-making precision. Even in the absence of discernible bias in external guidance, the act of conferring trust can engender uncertainties, influencing the overarching decision-making paradigm. This underscores the imperative of exercising discernment in allocating trust, particularly when the veracity of external guidance remains ambiguous or uncorroborated.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{Percentage_Principle_trustness_halfbias.pdf}
    \caption{}
    \label{fig:Percentage_Principle_trustness_halfbias}
\end{figure}
